Risk-Averse Finetuning of Large Language Models

We consider the challenge of mitigating the generation of negative or toxic content by the Large Language Models (LLMs) in response to certain prompts. We propose integrating risk-averse principles into LLM fine-tuning to minimize the occurrence of harmful outputs, particularly rare but significant events. By optimizing the risk measure of Conditional Value at Risk (CVaR), our methodology trains LLMs to exhibit superior performance in avoiding toxic outputs while maintaining effectiveness in generative tasks. Empirical evaluations on sentiment modification and toxicity mitigation tasks demonstrate the efficacy of risk-averse reinforcement learning with human feedback (RLHF) in promoting a safer and more constructive online discourse environment.

==> sections/icml24_rebuttal.tex <==
\section{General Rebuttal}
We extend our gratitude to the reviewers for their insightful comments, questions, and suggestions. It is encouraging to note the reviewers' recognition of the significance of our work in addressing the critical issue of toxicity mitigation in Large Language Models (LLMs) (Pb2n, BeEC). We are particularly pleased with the interest expressed in our approach of incorporating risk-averseness into LLMs and Reinforcement Learning from Human Feedback (RLHF) (Pb2n). The acknowledgment of the paper's technical quality (Pb2n), its clarity of writing (Pb2n), and the simplicity and accessibility of our idea (BeEC) further motivates our research endeavors. 

Following the positive feedback, we acknowledge that some of the concerns raised by reviewers bqXH and BeEC seem to stem from certain misunderstandings. Specifically, the critique regarding the incongruence of our motivation arises from a misinterpretation of the term ``risk'' in Risk Averse Reinforcement Learning (RARL). Reviewer bqXH is associating ``risk'' in RARL solely with the variability of costs and sensitivity to modeling errors. However, in contexts where rewards represent safety, RARL also interprets "risk" as encompassing the potential for adverse outcomes across episodes - effectively encapsulating a broader notion of ``risk'' \cite{chow2015risk, greenberg2022efficient}. In fact, the reviewer's referenced work \cite{chow2015risk} mentions CVaR, the objective adapted in our work, as possessing the ``ability to safeguard a decision maker from the ``outcomes that
hurt the most'' \cite{serraino2013conditional}''. This clarification underlines that our motivation aligns closely with the foundational principles of RARL, aiming to enhance LLM safety through a nuanced understanding of "risk". 

While we find Reviewer BeEC's comments to be more oriented towards general impressions rather than specific technical details, we believe addressing these concerns can enhance the clarity and accessibility of our research to a broader audience. Regarding Reviewer BeEC's observations, there appears to be a misunderstanding about the source of Eq. 4. Contrary to the reviewer's identification of this equation with Proximal Policy Optimization (PPO), it actually originates from a log-space controller introduced by \cite{ziegler2019fine}, as mentioned in the paper. Furthermore, contrary to Reviewer BeEC's concerns regarding reproducibility, we have provided comprehensive information on the code setup and computational requirements in Appendix C (pages 17-20) of our paper. As is generally the norm, to further enhance reproducibility and facilitate understanding, we intend to release the complete codebase following the paper's acceptance. Reviewer BeEC recommended conducting experiments using GPT-3.5, and reviewer Pb2n using GPT-4. However, it's important to note that GPT-3.5 and GPT-4, being extremely large proprietary models not openly available for research, pose significant monetary and compute challenges for use within academic contexts.

We are eager to engage with and address reviewers' points to improve our manuscript, and provide detailed rebuttal as follows. 

%\textcolor{blue}{Should we include a self/GPT4 critical analysis of the work}

\section{Rebuttal Reviewer bqXH}
\subsection{Weaknesses}
\paragraph{W1} \textit{The motivation for this method is incongruent. The proposed approach lacks a direct connection to model safety and harmlessness. The concept of "risk" in RARL and the "safety" concerns of LMs are distinctly different. In RARL, "risk" pertains to the variability of costs and sensitivity to modeling errors [1], whereas in LM alignment, "safety" involves avoiding harmful responses.}

\paragraph{Points to cover} 1. Disagree 2. Define Risk in both cases 3. Unify both cases

We would like to respectfully disagree with the reviewer here. In reinforcement learning (RL), specifically in risk averse RL, "risk" also refers to the potential for rare but highly undesirable outcomes or tail events \cite{greenberg2022efficient}. This could involve catastrophic failures, substantial negative rewards, or entering unrecoverable states. These tail events represent rare but potentially highly impactful negative outcomes that an RL system seeks to avoid. The reviewer's referenced work \cite{chow2015risk}, also mentions CVaR, the objective adapted in our work, as an objective possessing the ``ability to safeguard a decision maker from the ``outcomes that
hurt the most'' \cite{serraino2013conditional}''.  

In Language Model (LM) alignment, ``safety'' generally refers to avoiding harmful, unethical, or undesirable outputs from the language model, especially in response to prompts or inputs that could elicit such outputs ("unsafe inputs"). It is accurate to say that ``risk'' in LMs can similarly be thought of in terms of managing or avoiding extreme or ``tail'' events, which in this case would be unsafe outputs to unsafe (tail) inputs. Unsafe inputs refer to prompts that could lead the model to generate harmful, inappropriate, or undesirable content. Managing these risks involves strategies to identify, mitigate, or prevent the model from engaging with or amplifying such inputs or generating unsafe outputs. So in essence, the concepts of risk in RL and safety in LMs are related - they both aim to mitigate low-probability but high-consequence adverse events or outputs.


\paragraph{W2} \textit{The proposed method lack significant technical novelty. The paper primarily applies RARL to LM alignment without identifying specific challenges inherent in this application and addressing them accordingly. Although a soft-risk scheduler is introduced, its effectiveness remains uncertain.}

\paragraph{Points to cover} 1. Novel integration 2. New risk scheduler 3. Choice of risk metric - why the choice is more practical 4. Choice of objective - where did we decide to induce risk, and why? Just on rewards vs rewards+KL 5. Actor critic algorithm 

We would like to respectfully disagree here as well. 

\paragraph{Innovative Risk-Aversion Strategy} Introducing a risk-averse strategy to LLM finetuning, focusing on optimizing Conditional Value at Risk (CVaR), represents a significant contribution to enhancing the safety and ethical considerations of LLM deployment. By optimizing the risk measure of CVaR, RA-RLHF specifically targets the minimization of toxicity in rare events, a challenge not explicitly addressed by traditional RLHF methods. Our work is the first to introduce a nuanced understanding of `risk' in the context of content generation. %In our work, we introduce application of CVaR over a regularized RL objective, something that hasn't been studied before in the context of RL. %The integration of risk-averse principles in the Reinforcement Learning from Human Feedback (RLHF) framework, specifically tailored for Large Language Models (LLMs) is novel. %This is a significant technical novelty as it addresses the critical challenge of mitigating the generation of harmful content by LLMs, particularly focusing on rare but impactful negative outputs.

\paragraph{Challenges} Risk-Averse Reinforcement Learning (RARL) encompasses a spectrum of risk criteria, such as mean-variance, entropic risk measure, distortion risk measure, and Conditional Value at Risk (CVaR), among others. The exploration of CVaR within the realm of Large Language Model (LLM) fine-tuning for safety enhancement represents a novel selection. In our work, we implement CVaR in conjunction with a regularized reinforcement learning objective (reward + KL term) with an aim to learn a complex parameterized policy (LLM). This is an unprecedented setting in both RL and LLMs.  
%Risk Averse RL (RARL) is a broad term encompassing various risk criteria including mean-variance, entropic risk measure, distortion risk measure, conditional value at risk (CVaR), etc. The decision to study CVaR in the context of LLM finuetuning to establish safety is a novel choice in itself. In our work, we apply CVaR over a regularized RL objective with an objective to learn a complex parameterized policy, something that hasn't been studied before in the context of both RL and LLMs.

\paragraph{Methodological contribution and Potential Impact} Beyond the immediate application of creating safer LLMs, this work contributes to the broader field of machine learning by demonstrating how risk measures like CVaR can be integrated into the training process of complex models like LLMs. Our work additionally establishes a groundwork for exploring additional risk measures and criteria, such as the Entropic Value at Risk (EVaR), in the context of LLM safety and uncertainty quantification. 

\paragraph{Empirical results}
In our submission, we conducted a comprehensive evaluation of Large Language Models (LLMs) focusing on tasks related to sentiment modification and toxicity mitigation. This assessment utilized a diverse set of metrics to ensure a holistic understanding of model performance. Specifically, we measured:

1. The average environment reward on test dataset, as detailed in Table 2 (columns 2 and 5), to gauge average sentiment modification and toxicity mitigation. 

2. The finetuned models' performance across different input quality levels measured in quantiles with results included in Figures 1 and 2 (column 5) and Table 2 (columns 3 and 6).

3. The perplexity of input-output pairs (Table 2, columns 4 and 7), providing insight into the finetuned models' generation quality.

4. Shifts in distribution, depicted through visual histograms in Figures 1 and 2 (columns 1-4), highlighting changes in model output characteristics.

Our findings consistently show that the RA-RLHF model outperforms the standard RLHF approach across these evaluation metrics. While we observed a marginal increase in model perplexity for RA-RLHF, this can likely be attributed to the model undertaking more aggressive adjustments to satisfy the goals of sentiment modification and toxicity mitigation. Importantly, this increase in perplexity does not compromise model performance; in fact, the perplexity scores for Jigsaw-Gen remain lower than those recorded for the GPT-2 model, underscoring RA-RLHF's  superior performance in avoiding harmful outputs while maintaining effectiveness in generative tasks. 

%The proposed methodology has significant implications for the responsible deployment of LLMs, offering a pathway to reduce the risks associated with toxic content generation. Our work not only contributes to enhancing digital interactions but also establishes a groundwork for exploring additional risk measures and criteria, such as the Entropic Value at Risk (EVaR), in the context of LLM safety and uncertainty quantification. %Our work can not only help contribute to a more positive online environment, but, our work also lays foundation for studying other risk measures and criteria like Empirical Value at Risk (EVaR) and associated technical challenges that come with the new optimization objective. %and enhance the public's trust in AI technologies

%\textcolor{red}{It is not clear to me what reviewer means by "effectiveness" of soft risk scheduler} 

%Are we supposed to do the following? 

%- Emphasize the empirical evaluations presented in your paper that demonstrate the efficacy of the soft-risk scheduler. Point out how the experimental results on sentiment modification and toxicity mitigation tasks show that your method achieves superior performance in avoiding harmful outputs while maintaining effectiveness in generative tasks. This directly counters the reviewer's concern about the uncertainty of the soft-risk scheduler's effectiveness.

%- Highlight specific examples or data from the experiments that showcase the positive impact of the soft-risk scheduler on model performance, especially in the context of reducing the occurrence of toxic outputs.

%- Highlight that finetuning an LLM with a soft-risk approach and constant batch size reduction based on the risk target are innovative methods specifically designed to address the challenge of good tail input performance in LLMs. 

%- Emphasize the broader impact of your work on fostering a safer and more constructive online discourse environment. Explain how the proactive stance of LLMs, as enabled by your methodology, in moderating content not only mitigates the risks of harmful language but also contributes to the advancement of responsible AI development.

\paragraph{W3} \textit{The experimental evidence provided is not convincing. The datasets IMDB-Gen and Jigsaw-Gen only cover two narrow tasks that are not inherently designed to evaluate the harmlessness and helpfulness of LMs. Additionally, the absence of reliable metrics regarding response quality is notable. Furthermore, the proposed method could perform worse than all baselines in some cases, as indicated in Table 2.} 

\paragraph{Points to cover} 1. Study of generative tasks is the first method anybody doing a systematic research would try. 2. Why have we moved away from HH paradigm? . 3. Justify current metrics - explain how they are complete in assessing what we want to test. 4. Write all the inferences from Table 2 clearly. 

Our research introduces a nuanced perspective on inducing safety in large language model (LLM) outputs, even encompassing characterization of safety through dual-axis approach of assessing helpfulness and harmlessness independently \cite{bai2022training, ganguli2022red}. The work by \cite{bai2022training} introduces the concepts of helpfulness and harmlessness, noting best performance tradeoff on LLMs RLHFed with a preference model (PM) trained on the combined HH dataset (see Fig. 1 in \cite{bai2022training}). They mention ``fortunately, we find that PMs trained on a mixture of both datasets can nevertheless learn the right lessons and behave helpfully when appropriate,
while encouraging the polite refusal of harmful requests''. In both \cite{bai2022training, ganguli2022red}, characterization of safety is done through a single reward/preference model, as is the case in our work. We, in fact, demonstrate in our work how the RLHF finetuning process can be made risk-averse using risk averse principles, algorithmically going beyond what is established in \cite{bai2022training, ganguli2022red}.

More recently, the work by \cite{dai2023safe} introduces Safe-RLHF requiring separate models to evaluate the helpfulness and harmlessness of responses. This dual-model framework adds complexity to the safety induction process, necessitating the management of two distinct assessment criteria. In contrast, as mentioned above, we work with a single reward model. This singular reward-based framework is particularly advantageous when the reward model is tuned to accurately reflect safety considerations specific to the task at hand. Under such circumstances, RA-RLHF can effectively navigate the safety landscape, ensuring that LLM generations meet the desired standards without the need for dual evaluations. This consolidation into a single reward model offers a more efficient and potentially more effective mechanism for achieving safe and reliable LLM outputs across broader applications. %In contrast, our work proposes a unified strategy by employing a single, comprehensive reward model that can encapsulate both the helpfulness and harmlessness dimensions into a singular safety metric. %In a lot of downstream tasks, enterprise or otherwise, it is operationally much easier to work with a single preference model. %Our work thus reduces the operational complexity associated with maintaining separate models for helpfulness and harmlessness. %By integrating both criteria into one cohesive reward function, our risk-averse reinforcement learning with human feedback (RA-RLHF) method optimizes LLM outputs for overall safety, ensuring that generated responses are not only beneficial but also devoid of harmful content.

%of both helpfulness and harmlessness

Additionally, our selection of IMDB-Gen and Jigsaw-Gen tasks for evaluating our method is grounded in the scientific approach of progressive investigation. These tasks, while specific to generation, are critically relevant for assessing the fundamental capabilities of LLMs in generating content that is both non-toxic and contextually appropriate. By focusing on these generation tasks, we aim to establish a solid foundation upon which more complex applications, such as conversational AI, can be built. This is a standard practice in the field, allowing for focused analysis before extending to broader contexts.

%Having said that, we do acknowledge the reviewer’s point regarding the need for diverse tasks to evaluate harmlessness and helpfulness comprehensively. However, as the first study to explore risk-averseness in RLHF, our work initiates a critical discourse on integrating safety principles into LLM fine-tuning. Our approach demonstrates a novel methodology for reducing harmful content generation, a significant step towards the broader goal of enhancing LLMs’ harmlessness and helpfulness.

Having said that, we recognize the importance of continuous improvement and the expansion of our methodological framework to cover a broader range of tasks. Our work lays the groundwork for future studies to explore and refine the integration of risk-aversion in LLM fine-tuning.

%\textcolor{red}{I don't understand the comment about metric. Do they mean separate help and harm scores instead of a single reward?}

%\textcolor{red}{By relation to baselines, do they mean variance in results?}


\subsection{Questions}
\paragraph{Q1} \textit{Why do the x-axis scales and number of bins in Figure 1 looks different for different methods?} 

Thank you for pointing out the difference in x-axis scale for Fig.1, column 1 which reports prompt scores. In the original Fig. 1 included in the submission, the scale is the same for all the finetuning methods - SFT, RLHF and RA-RLHF. The bin size is the same as well. We have now included an adjusted x-axis scale column 1 in Fig. 1. 

\paragraph{Q2} \textit{This paper use Jigsaw Toxicity Classification dataset in an unintended way. It employs the dataset to finetune a generation model for completing comments, despite the reward model primarily targeting the identification and penalization of toxic content. Further elucidation regarding the modifications made to the dataset is warranted.}

\paragraph{Points to cover} 1. How does inclusion of Jigsaw make our evaluation diverse - in terms of dataset having different properties than IMDB (data distribution wrt reward, etc) 2. Clarification on use of reward model - in both IMDB and Jigsaw - both tasks use reward model in exactly the same manner. 

In our work, both IMDB and Jigsaw datasets are used to source prompts for generation. Usage of Jigsaw dataset to source prompts for generation is indeed novel, paralleling how IMDB dataset is utilized for generation in \cite{ramamurthy2022reinforcement}. This adaptation involves no alterations to the dataset's content. Additionally, these datasets come with public reward models, making them a suitable choice in RLHF settings. Finetuned LLMs maintain good language generation capabilities by virtue of being tethered to the base model through a KL term. So, reward models need to only serve the purpose of inducing preferences, which in our case means evaluating generations over sentiment (in case of IMDB), and toxicity (in case of Jigsaw). Thus, our approach demonstrates the Jigsaw dataset's utility beyond its original classification purpose, contributing to the broader goal of minimizing harmful online content.

%From paper: Ramamurthy et al. (2022) transformed this task into IMDB-Gen by prompting an LLM with a movie review’s beginning and tasking it to complete the review aiming for maximal positive sentiment. In contrast, the Jigsaw Toxicity Classification involves discerning and categorizing toxic comments, such as threats, obscenity, insults, and identity hate. We propose its generative version, Jigsaw-Gen, that tasks an LLM with continuing a prompt in the least toxic manner possible

\section{Rebuttal for Reviewer Pb2n}
\subsection{Weaknesses}
\paragraph{W1} \textit{Although this paper provides experimental evaluations on two language generation tasks on IMDB sentiment classification and Jigsaw toxicity classification, this work would have bigger impact if the authors could adopt the ideas and methods to large scale real problems, for example, language generation for conversational AI and so on.} 

\paragraph{Points to cover} 1. Study of generative tasks is the first method anybody doing a systematic research would try. 2. Say how conversational AI is a subset of generation - where the type of input changes from one sentence/phrase to a conversation up until a point. 3. Say conversational AI can be future work. 

Our selection of IMDB-Gen and Jigsaw-Gen tasks for evaluating our method is grounded in the scientific approach of progressive investigation. These tasks, while specific to generation, are critically relevant for assessing the fundamental capabilities of LLMs in generating content that is both non-toxic/well-sentiment-ed and contextually appropriate. By focusing on these generation tasks, we aim to establish a solid foundation upon which more complex applications, such as conversational AI, can be built. In fact, conversational AI is a special case of content generation where the type of input changes from one sentence/phrase to a conversation up until a point. %This is a standard practice in the field, allowing for focused analysis before extending to broader contexts. \textcolor{blue}{add citations}

\subsection{Questions}
\paragraph{Q1} \textit{We are curious that what are the results if the authors use other powerful LLMs as pre-trained models and baselines for comparison, for example, GPT4, Llama2, Mixtral and so on.}

\paragraph{Points to cover} 1. Include results with GPT-J-6B. 2. Explain compute requirements and feasibility with larger models. 3. Possibly more data needed with larger models? 

GPT4 is a $\sim1.8$ billion parameters model with storage requirement of $\sim750$ GB, and is not open source. Mixtral is a mixture of $8$ $7$B parameters models requiring $\sim 96.8$ GB storage. Study of these models in academic contexts is challenging because of large compute requirements and long training times. For example, while RLHF-finetuning a model with 7B parameters in 16 Bit precision with AdamW, the storage requirement for the model is 8 bytes per model parameter - a number that comes upto 56GB without accounting storage for forward activations, temporary memory, data and functionality specific memory {Include HF reference}. Additional 14GB+ is required for the reference model. This makes it impossible to finetune llama 7B even on an A100 80 GB GPU. 

We would also like to highlight that many of the recent works making algorithmic contributions like Direct Preference Optimization (DPO) \cite{rafailov2024direct} use relatively smaller sized models for experimental evaluation like GPT2 and Pythia-2.8B. 

Having said that, we conducted additional experiments on the IMDB-Gen task using a GPT-J-6B model, and have added the same in the appendix.  

\paragraph{Q2} \textit{In experiment part, what is the scalability of the datasets?}
\textcolor{red}{Does it mean how our approach would perform with larger data sizes?}

\paragraph{Points to cover} 1. Mention our dataset sizes, and how they compare to other datasets in the generation/conversational AI space. 2. Include results on a larger dataset (Real toxicity prompts 57.9k train size)?  

We're not quite sure what you mean by scalability of the  dataset. Assuming you mean mean how our approach would perform with larger sized datasets, we added another task based on the RealToxicityPrompts dataset. RealToxicityPrompts-Gen has a training size of 57.9k prompts compared to IMDB's 25k and Jigsaw's 36.9k. The results are detailed in section F.1 and F.1.1 in the appendix and we observe that once again RA-RLHF does a better job in generating text continuations with minimized toxicity levels.
% Its worth noting that in ths task, SFT model performs worse than the zero shot model due to likely mismatch in Perspective APIs evaluaton of toxicity as compared to Unitary's ToxicBERT model. Nonetheless, RA-RLHF manages to shift the distrition further right than RLHF. 
\paragraph{Q3} \textit{In Fig.3(a), it seems that the reward curve of RA-RLHF is not convergent yet? In Fig.3(c), it seems that RA-RLHF does not have significant improvement of rewards compared to RLHF.}

Thank you for your question. We have run the training for both the tasks till the model goes over the entire dataset once. The plots correspond to the same. We did observe more gain in terms of environment reward for the IMDB-Gen task than the Jigsaw-Gen. We attribute this to the overall toughness of the task. Jigsaw-Gen contains highly toxic prompts that are generally tougher to counter with positivity even for humans - as observed by our own qualitative evaluation of the prompts and the responses. 

\section{Rebuttal for Reviewer BeEC}
\subsection{Weaknesses}
\paragraph{W1} \textit{The evaluation is weak, as there are only two datasets covering only two language generation tasks. Also, this work only uses GPT-2 as the base model in the evaluation. We are not sure if this method can be widely applied to other LLMs.}

\paragraph{Points to cover} 1. Explain compute requirements and feasibility with larger models. 2. Possibly more data needed with larger models? 

Our selection of IMDB-Gen and Jigsaw-Gen tasks for evaluating our method is grounded in the scientific approach of progressive investigation. These tasks, while specific to generation, are critically relevant for assessing the fundamental capabilities of LLMs in generating content that is both non-toxic/well-sentiment-ed and contextually appropriate. By focusing on these generation tasks, we aim to establish a solid foundation upon which more complex applications, such as conversational AI, can be built. In fact, conversational AI is a special case of content generation where the type of input changes from one sentence/phrase to a conversation up until a point.

\paragraph{W2} \textit{The reproducibility is inadequate, since there is no code released or included in the supplementary materials.}

%\textcolor{red}{This is no ground for rejection. Most papers release code upon acceptance. We will release the code upon paper acceptance.}

We would like to point the reviewer to Appendix C (pages 17-20) of our paper where we provide comprehensive information on the code setup and computational requirements. Also, as is generally the norm, to further enhance reproducibility and facilitate understanding, we intend to release the complete codebase following the paper's acceptance. 

\paragraph{W3} \textit{The presentation needs to be improved. For example, the authors can cut down the preliminaries and leave more blank to analyse the results. Some equations like Eq. 4 should already exist in Proximal Policy Optimization (PPO) and authors can mention it and connect it to PPO, rather than write them down again.}

We would like to point to the reviewer that their identification of Eqn. 4 as coming from Proximal Policy Optimization (PPO) is incorrect. It actually originates from a log-space controller introduced by \cite{ziegler2019fine}, as mentioned in the paper. Eqn. 4 is an important detail to explain the RLHF setup used in our work. We have not included any policy gradient equation from PPO in our work to keep the manuscript concise.

\subsection{Questions}
\paragraph{Q1} \textit{Can authors present more experimental results on other LLMs with different sizes like GPT-3.5, LLaMA or Vicuna?}

GPT4 is a $\sim1.8$ billion parameters model with storage requirement of $\sim750$ GB, and is not open source. Mixtral is a mixture of $8$ $7$B parameters models requiring $\sim 96.8$ GB storage. Study of these models in academic contexts is challenging because of large compute requirements and long training times. For example, while RLHF-finetuning a model with 7B parameters in 16 Bit precision with AdamW, the storage requirement for the model is 8 bytes per model parameter - a number that comes upto 56GB without accounting storage for forward activations, temporary memory, data and functionality specific memory {Include HF reference}. Additional 14GB+ is required for the reference model. This makes it impossible to finetune llama 7B even on an A100 80 GB GPU. 

We would also like to highlight that many of the recent works making algorithmic contributions like Direct Preference Optimization (DPO) \cite{rafailov2024direct} use relatively smaller sized models for experimental evaluation like GPT2 and Pythia-2.8B. 

Having said that, we conducted additional experiments on the IMDB-Gen task using a GPT-J-6B model, and have added the same in the appendix.  

\paragraph{Q2} \textit{Would you like to present more analyses on the results, to show that this method can successfully mitigate generating toxic content?} \textcolor{red}{Is there any other analysis on existing results that we can add in appendix?}

In our submission, we conducted a comprehensive evaluation of Large Language Models (LLMs) focusing on tasks related to sentiment modification and toxicity mitigation. This assessment utilized a diverse set of metrics to ensure a holistic understanding of model performance. Specifically, we measured:

1. The average environment reward on test dataset, as detailed in Table 2 (columns 2 and 5), to gauge average sentiment modification and toxicity mitigation. 

2. The finetuned models' performance across different input quality levels measured in quantiles with results included in Figures 1 and 2 (column 5) and Table 2 (columns 3 and 6).

3. The perplexity of input-output pairs (Table 2, columns 4 and 7), providing insight into the finetuned models' generation quality.

4. Shifts in distribution, depicted through visual histograms in Figures 1 and 2 (columns 1-4), highlighting changes in model output characteristics.

Our findings consistently show that the RA-RLHF model outperforms the standard RLHF approach across these evaluation metrics. While we observed a marginal increase in model perplexity for RA-RLHF, this can likely be attributed to the model undertaking more aggressive adjustments to satisfy the goals of sentiment modification and toxicity mitigation. Importantly, this increase in perplexity does not compromise model performance; in fact, the perplexity scores for Jigsaw-Gen remain lower than those recorded for the GPT-2 model, underscoring RA-RLHF's  superior performance in avoiding harmful outputs while maintaining effectiveness in generative tasks.  

\paragraph{Q3} \textit{Can this method be applied to other policy optimization algorithms like Direct Preference Optimization (DPO)?}

Since we build upon RLHF, we require a reward model to induce risk-averseness. DPO, on the other hand, works with datasets without an explicit notion of rewards. To characterize risk averseness in DPO like objectives is an interesting problem, and left for future work. 


\section{Experiments}
\begin{itemize}
  \item GPT-J-6B for IMDB and Jigsaw.
  \item RealToxicityPrompts task
  \item BeaverTails task (w/ BeaverCost as reward model and BeaverReward as perplexity equivalent)
  \item Regenerate Fig 1 with same X-axis
\end{itemize}

\bibliography{example_paper}
\bibliographystyle{icml2024}

==> sections/introduction.tex <==
\section{Introduction}
The deployment of large language models (LLMs) is witnessing a remarkable growth across both personal and professional domains.  While a majority of users utilize LLMs via relatively innocuous prompts, a minority might do so with negative or toxic prompts, leading to generation of content that violates acceptable norms.  It is these rare, toxic outputs, which, when virally spread via social media could result in a negative perception of LLMs as a whole and so restrict their use in innovative applications with broad societal impacts.  Can LLMs be finetuned to avoid such outputs?

A recent approach to finetuning LLMs is via reinforcement learning with human feedback (RLHF), using labelled data collected from human experts.  A natural extension is the idea of constrained or ``safe'' RL as applied to LLM finetuning, which optimizes the reward, while constraining the \emph{expected} harmfulness score of the output to be within limits~\cite{dai2023safe}.  However, the notion of constraining expectation simply implies that the scores of positive trajectories could cancel out those of the negative trajectories---not explicitly constrain the probability of such toxic outputs occurring in the first place.  How are we to ensure that rare, but high-stakes event probabilities are minimized?

The key idea that we explore in this work is to bring the notion of \emph{risk-averseness} into the realm of LLMs.  Unlike the traditional RLHF, which seeks to maximize the expected reward in a risk-neutral manner, we seek to optimize a risk measure of the generated trajectories.  The specific measure that we use follows Conditional Value at Risk (CVaR), which minimizes the expected cost, conditioned on it being greater than a certain quantile value $\alpha$~\cite{tamar2015policy,greenberg2022efficient}.  In other words, we seek to minimize the toxicity or negativity, specifically of rare events that might occur.

\input{sections/main_results}

Our objective is to develop a risk-averse RLHF (RA-RLHF) algorithm to utilize pre-collected prompts and their associated responses, which have varying levels of negativity or toxicity, to finetune an LLM to be risk-averse.   Several ideas need to come together to realize such an approach.  The two elements that must be considered during each policy iteration step is the the risk-level quantile that we train against in that step, and the batch size of data to be used in that step. We use a \emph{soft-risk} approach during the initial training period, wherein we set only small risk levels and utilize the entire data so that the policy learns to produce successful outputs (not just non-toxic ones) in the manner of~\citet{greenberg2022efficient}.  We then train with a constant rate of batch size reduction, based on the risk target, to enable the policy to focus on hazardous prompts with the worst returns.   These two elements, when coupled with a  supervised finetuned base-policy that we regularize against, produces policies that not only display risk-aversion when exposed to negative or toxic prompts, but actually perform better than a traditional RLHF-tuned policy over all prompts.

Our nominal use-case is to enable the capability to not only generate responses to queries, but also modify or propose real-time adjustments to content that verges on being inappropriate.  For instance, consider a scenario on a social media platform such as Reddit.  When a user initiates potentially offensive content, the LLM can intervene by generating alternatives or suggestions that could steer the conversation away from toxicity.  These prompts are rare but significant, occupying the tail of a distribution measuring non-toxicity of rewards, which are well addressed by our risk-averse approach.   This proactive stance of LLMs in moderating content not only mitigates the risks of harmful language but also fosters a more positive and respectful online discourse.

We evaluate the performance of RA-RLHF under two such language generation scenarios, using GPT2 as the base LLM.  The first task, which follows  \citet{ramamurthy2022reinforcement} pertains to an IMDB data set, where the LLM is provided with the initial part of a movie review, which acts as the prompt, and could have either a positive or negative sentiment.  The LLM is tasked to coherently complete the review to ensure a positive sentiment.  We also created a second task using the Jigsaw dataset, which contains text samples with different levels of toxicity, insults, hate, and so on.  Again, we create a prompt with the initial part of the text, and the generative model is tasked with completing the text in a non-toxic manner.  The outputs in each case are evaluated using a standardized scoring model.

Figs.~\ref{fig:imdb-dist-shift}-\ref{fig:jigsaw-dist-shift} provide performance illustrations.  The first graph on the left shows the prompt data distribution in terms of sentiment or toxicity for the two tasks. The next shows the performance of supervised fine-tuning (SFT) over the positive/non-toxic data to obtain a finetuned LLM, which generates language consistent with the task type.    The next two show the output distributions of RLHF, which attempts to maximize the expected reward, and RA-RLHF, which is risk-averse.  The relative benefits of RLHF vs. RA-RLHF can be seen in the final graph, where we order the prompts in decreasing order of negativity/toxicity, i.e., the left side is the riskiest prompt quantile.  We observe that RA-RLHF not only dominates over RLHF, it also does so specifically in the riskiest quantiles where the generative tasks are hardest.  Table~\ref{tab:generations} provides examples of the prompts and the corresponding outputs for both task types.  Again, we notice that RA-RLHF is particularly good at steering the language in the right direction when exposed to negative/toxic prompts.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In the contemporary digital landscape, the deployment of large language models (LLMs) is witnessing a remarkable growth across both personal and professional domains. Our work concentrates on the innovative application of generative content moderation within the realm of social media. Traditionally, content moderation on social media platforms is approached as a classification task \cite{singhal2023sok}. However, the increasing utilization of LLMs in this context marks a significant shift in methodologies.

% Our focus in this work is on soft content moderation by transforming the task of content moderation from a mere classification into generative one. This transition represents a groundbreaking method in applying language models to digital content management. Unlike the conventional approach of simply categorizing content as either acceptable or unacceptable, a generative model offers a more dynamic solution. It possesses the capability to not only identify but also modify or propose real-time adjustments to content that verges on being inappropriate.

% For instance, consider a scenario on a social media platform such as Reddit. When a user initiates potentially offensive content, the LLM can intervene by generating alternatives or suggestions that could steer the conversation away from toxicity. This proactive stance of LLMs in moderating content not only mitigates the risks of harmful language but also fosters a more positive and respectful online discourse.

%%%We live an era of ever increasing large language model usage for both personal and business use. In this work we focus on the application of generative Content Moderation in Social Media. Content Moderation in Social Media is generally viewed as a classification task, and large language models (LLMs) are increasingly being used for this task. Transforming classification tasks into generative tasks offers a novel approach to handling language model applications. Instead of just classifying content as appropriate or inappropriate, a generative model could be used to actually modify or suggest instantaneous modifications to borderline content. For example, when a user begins writing something offensive on a platform like Reddit, the LLM can produce generations that can potentially sway the user towards nontoxicity. %However, language modeling applications, like those in autonomous driving, healthcare treatment planning, financial trading, and robot control, involve a delicate balance between reward and reward.

% Addressing the complex challenges posed by user initiations/prompts in social media requires an advanced level of discernment by language models. Such prompts may necessitate a nuanced comprehension of context, the ability to interpret language subtleties such as sarcasm or humor, and an awareness of cultural sensitivities. These prompts are rare but significant, occupying the tail of a distribution measuring non-toxicity rewards. To investigate and effectively respond to these outlier events, we propose usage of risk-aversion techniques in LLM alignment before deployment. This strategy is designed to optimize the model's performance on these less frequent but critical instances, thereby enhancing the overall robustness and reliability of the content moderation system.

%%%What becomes especially tricky in this scenario is to perform well on user prompts that can require, amongst other things, a sophisticated understanding of context, language nuances like sarcasm/humor, and cultural sensitivities. If we were to plot a distribution over non-toxicity reward for all the prompts, these prompts would lie in the tail of this distribution. To study these tail events we take the route of risk-averse reinforcement learning. 

% To study and perform well on these tail events, we make use of the framework of language generation as a token level Markov Decision processes (MDP). We aim to induce good generations using reinforcement learning from human feedback (RLHF). To do especially well on tail events, we borrow ideas from Risk-averse reinforcement learning (RL) algorithms that aim to learn RL policies that perform well on the worst set of environment conditions \cite{ tamar2015policy,greenberg2022efficient}. In the context of language generation, such environment conditions correspond to the input contexts that fall under `risky' tail described above. 

% keep it here, so that main results appear on page 2


%For example, in machine translation (MT), the reward is achieving accurate and fluent translation across languages. The risk involves cultural insensitivity or inaccuracies, especially in contexts where nuances and local idioms are important. Poor translation can lead to misunderstandings or offense, particularly in diplomatic or international business contexts. Similarly, in situations where language models are used to moderate content on social media platforms, the challenge is to maximize the removal of harmful or inappropriate content (reward) while minimizing the risk of erroneously censoring legitimate content (risk). An overly aggressive model might restrict free speech or suppress important discussions, while a lenient model could fail to catch harmful content, affecting user experience and potentially causing legal issues.

%%%%%%%%%%%%%%%


% \redtext{Make a case for smaller application specific finetuned models. Should we include results from quantized trained models? Make a case for use of or work to inspire further research in this space. 

% LLMs used for lower level control. 

% \paragraph{Risks in Language Modeling}

% "this is a great movie. I love the series on tv and so I loved the movie. One of the best things in the movie is that Helga finally admits her deepest darkest secret to Arnold!!! that was great. i love"

% An important aspect of our work is to define what risk means in language modeling tasks. We need to clarify the context in which we are using the word risk. It is not the societal-risk from using LLMs (like in: https://arxiv.org/pdf/2112.04359.pdf, https://cltc.berkeley.edu/2021/08/03/ai-language-models-mitigating-harms-through-responsible-research-and-publication/). But, risk of performing poorly on certain critical inputs. The risky events in our case are the inputs on which our models don't perform well on? For example for IMDB generation task, why doesn't the RLHFed model work well for certain test inputs. 

% In this spirit, we can discuss the following things here: 
% \begin{enumerate}
%     \item Consider the SFT+PPO RLHFed model. Perform generation on all the test inputs using this model. Across three different input and output lengths, plot the distribution of rewards. Identify tail inputs from these. 
%     \item Analyse tail event inputs and generations. Neatly include tail event examples. 
% \end{enumerate}

% % \begin{figure*}[ht!]
% %     \centering
% %     \includegraphics[width=\textwidth]{icml2024/figures/risk_llm/risk_fig_1.png}
% %     \caption{Studying risky datapoints of the IMDB dataset.}
% %     \label{fig:exp_1}
% % \end{figure*}

% Comment on bias in reward/preference model, and how that might affect inferences. 
% }



